A First Look at COVID-19 Messages on WhatsApp in Pakistan

The worldwide spread of COVID-19 has prompted extensive online discussions, creating an `infodemic' on social media platforms such as WhatsApp and Twitter. However, the information shared on these platforms is prone to be unreliable and/or misleading. In this paper, we present the first analysis of COVID-19 discourse on public WhatsApp groups from Pakistan. Building on a large scale annotation of thousands of messages containing text and images, we identify the main categories of discussion. We focus on COVID-19 messages and understand the different types of images/text messages being propagated. By exploring user behavior related to COVID messages, we inspect how misinformation is spread. Finally, by quantifying the flow of information across WhatsApp and Twitter, we show how information spreads across platforms and how WhatsApp acts as a source for much of the information shared on Twitter.

==> Drafts/char_misinfor.tex <==
\subsection{Characterizing Misinformation}

\gareth{This seems an odd title, as the previous sections have also been characterizing misinformation?}

\begin{figure}[h]
    \centering
    \includegraphics[width=.45\textwidth]{wa_images_timeseries.pdf}
    %\includegraphics[width=8cm, height=6cm, keepaspectratio]{perdayStats.png}
    \textbf{ \caption{\textbf{Percentage of types of COVID-19 daily images shared between 16 March and 09 April.} \label{fig:COVID-19 Images Tagged}}}
\end{figure}


As discussed above, misinformation tends to spread rapidly via WhatsApp. This can be observed in Figure \ref{fig:COVID-19InformationvsMisinformation}. Out of the 1995 COVID related images analyzed, 11\% of the images were classified as misinformation. We saw a rapid rise in misinformation up to 19 March, and since then a diminishing trend is observed. The decrease can be attributed to government, news channels, religious clergy and civil society starting various campaigns to tackle misinformation.\footnote{\url{https://www.arabnews.pk/node/1644161/pakistan}} The effects of campaign can be clearly seen in our data, as there is a high influx of health information related to the pandemic appearing over time, while misinformation decreases. This is an encouraging trend, which solidifies that the methods taken to tackle misinformation are working.

    
\begin{figure}[h]
    \centering
    \includegraphics[width=.45\textwidth]{misinfo-example.png}
    %\includegraphics[width=8cm, height=6cm, keepaspectratio]{perdayStats.png}
    \textbf{\caption{\textbf{Examples of misinformation.} \emph{a) A fake medicine that is said to cure Corona, b) fake method of combating COVID-19, c) a fabricated quote associated with a provincial health minister, d) Another fabricated quote, this time, with a news channel look.}}\label{fig:COVID-19ExampleofMisinformation}}
\end{figure}


    
\kiran{This is probably the most interesting contribution of the paper. So we should focus and dig deeper into this. Can we analyze the images for the rest of the duration as well (also in April)? At least for a sample?}
\ignacio{Agree. We could also split by types of messages/groups wrt language, political party (to which the channel is related to), country-code (or prevalence of specific/non-Pakistani country codes in a given group). Would be particularly interesting to see whether there are different patterns wrt intensity and precedence (ie, which groups/users lead in time in the sharing of misinformation)}


\subsubsection{Types Of Misinformation}

We saw various types of misinformation, ranging from fabricated headlines to fake facts about COVID-19. In order to understand the misinformation being spread, we categorized it as following 1) Treatments, prevention and causes, 2) Fabricated news, like deaths in Italy taken out of context, 3) Fabricated quotes, attributed to popular personalities, which they never said. It was observed that the main medium of misinformation is via doctored images of popular TV channel news bulletins. As a result the receiving audience tends to accept these images with much more credibility. Furthermore, images of popular personalities, political, social and even journalists are also used to add credibility to the contents shared within an image. Figure \ref{fig:COVID-19ExampleofMisinformation.} shows various popular ways misinformation is spread on WhatsApp.
\gareth{Could we quantify/evidence some of the above statements?}


After manually tagging the images, it was found that 45.5\% of the misinformation shared was related to fake treatments, prevention and causes of COVID-19. Fabricated news amounted for 35.7\% of the misinformation, whereas 18.8\% of the misinformation was of fabricated quotes.

\gareth{This section seems a bit unexpected, as it mashed together parts of misinformation that have been touched upon earlier in one way of the other}

\subsubsection{Relation With Health Information}
An interesting take from this is how misinformation seems to be independent of the influx of health information. But in reality that is not the case and both of them are interconnected. Since users have a tendency to share snippets of news articles and headlines, as a result the information propagated through electronic and print media, tends to show up on WhatsApp with a delay. As a result, users were exposed to awareness campaigns and resulted in reduced misinformation on WhatsApp. Whereas at the same time, it took time for the new ads, campaigns to come to WhatsApp, as users tend to create images from other content. Hence instead of overall declaring misinformation and health information, the decrease in misinformation happening a day earlier than the influx of health information, can be attributed to this behaviour.  \gareth{This needs more quantification. Could we talk about how the spread of this differs to other groups of misinformation?}

\subsubsection{Religion}
The importance of religion, within the Pakistani community, can be seen in the fact that 23\% of the average images shared by users were religious in content. That means that out of every 5 images shared, 1 was inspired by religion. Within our chosen time frame, a critical COVID-related religious debate started within Pakistan, whether to stop the compulsory Muslim congregational prayers in mosques\footnote{https://www.dw.com/en/coronavirus-and-islam-pakistani-clerics-refuse-to-shut-down-mosques/a-52969639} or not. As a result from 23 March onward, a constant increase in religious traffic can be observed.

%\begin{figure}[h]
%    \centering
%    %\includegraphics[width=.5\textwidth]{perdayStats.png}
%    \includegraphics[height=5.8cm, %keepaspectratio]{AverageGroupContentType.png}
%    \textbf{ \caption{Type of content shared on average, daily, in the top 10 %groups.} }
%\end{figure}

%\gareth{Would be good to have some more user-centric analysis here, which looks at how individual users are repsonible for spreading content across groups. Could you also do some temporal analysis to estimate if there are people who copy content across | TJ: Adding PDQ to find temporal propagation of images.}



\gareth{Overall I think this section needs a strong narrative linking together the sections. At the moment, they read like a disconnected set of short sections. Ideally, we could spin them into more or a coherent story. I've tried to put some linking text, but I reckon it needs a bit more further work.}

==> Drafts/data_characterization.tex <==
\section{Data Characterization}

\kiran{I think we dont need to separate the characterization to the dataset description. a lot of my questions can be answered by merging them.}
We start by presenting a brief characterization of our dataset. An overview of the messages collected from the 227 public groups (January 10 up till April 20) is shown in Table \ref{table:dataset_overview}. The groups were joined over some time during this period. \gareth{Over how long is this spread? I guess we have some groups that we've joined for months, and others that we have only joined for days/weeks? Could we quantify this briefly.}
These groups are joined by 18,000 users, of which 89\% are unique (i.e., they only are present in a single group).
\ignacio{whatassp groups are politically related, but we do not characterise Pakistan's political landscape (number of parties/voters, ideological/religious spectrum, regional/national) nor map the groups to them -do we have more users/messages from a particular region and/or political/religious preference?}


\begin{table}[hbt]
\textbf{ \caption{ \textbf{Dataset Overview} } \label{table:dataset_overview} }
\begin{center}
\begin{tabular}{| r | c | c | }
\hline
\#Groups    &    227 & \\
\hline
\#Admins	& 521  & \\
\hline
\#Users    & 18475  & \\
\hline
\#Unique Users &	 16493 & \\
\hline
Total \#Messages  &    122876 & \\
\hline
\ & \\
\hline
\#Texts     &    58897 & 48.0\% \\
\hline
\#Images    &    31328 & 25.5\% \\
\hline
\#Video     &    20920 & 17.0\% \\
\hline
\#Audio     &    4991 & 4.0\% \\
\hline
Others      &    6740 &   5.5\%\\
\hline
\#URLs  &    14836 & \\
\hline
\#Unique URLs   &    8811 & \\
\hline
\end{tabular}
\end{center}
\end{table}


\begin{figure}[htb]
    \centering
    \includegraphics[width=8cm]{content_trend.png}
    \caption {\textbf{Type of content from 10 Jan to April 20.} \emph{Content: 49\% Texts, 25\% Images, and 16\% Videos}\ignacio{may be have 2 figures one for covid related and one for not related}}
    \label{fig:content_trend}
\end{figure}

Figure \ref{fig:content_trend} shows the number of texts, images, video, and audio messages shared over the course of our data collection. Text messages are the most utilized means of information dissemination in these groups constituting 48\% of all messages, followed by images, videos, and audio messages with 25.5\%, 17\%, and 4\% shares respectively. Figure \ref{fig:content_trend} shows this trend is followed but the ratio of the types of messages (texts, images, etc) is not consistent. For a brief period, text messages constitute an even larger than the average 49\% portion of all shared content as visible in Figure \ref{fig:content_trend}. 5.5\% of messages are labelled as ``Others". 50\% of them are PDFs and the rest consist of GIFs, Vcards, Deleted Messages etc.
%  \gareth{As it does not add up to 100\%, where type are the other posts? I'm guessing they're not all vcards etc? Are they files?}


\subsection{Location of Users}
Figure \ref{fig:users_map} shows the number of users that have joined our target groups by country. The country code at the start of a group members' number is used to extract this information. Table \ref{table:user_locations} summarizes the top 10 countries based on their number of Users.\ignacio{are there groups dominated by Pakistani expatriates in a particular country? if so worth checking whether they are more affected by local than Pakistani dynamics}

\begin{table}[hbt]
\textbf{ \caption{ \textbf{Locations of User by Country (Top 10).} \emph{91\% from Pakistan, 9\% from other Countries} } \label{table:user_locations} }
\begin{center}
\begin{tabular}{ | r | c | c | }
\hline
\textbf{Country}    &    \textbf{\#Users} &  \\
\hline
Pakistan    & 15068 & 91.0\%\\
\hline
India    & 495  & 3.0\%\\
\hline
Saudi Arabia & 223 & 1.3\%\\
\hline
United Arab Emirates & 182 & 1.1\%\\
\hline
United Kingdom & 55 & 0.3\%\\
\hline
Indonesia & 55 & 0.3\%\\
\hline
Nigeria & 40 & 0.24\%\\
\hline
United States & 32 & 0.19\%\\
\hline
Iran & 25 & 0.15\%\\
\hline
Australia & 24 & 0.14\%\\
\hline
Other & 294 & 1.78\%\\
\hline
\end{tabular}
\end{center}
\end{table}

Our candidate groups with 16k unique users being of Pakistani origin, consist of 91\% Pakistani users. Followed by around 500 users from India, few hundred from Middle Eastern States (Saudi Arabia, United Arab Emirates), two digit users from UK, Indonesia, Nigeria, USA, Australia, and Iran. It may be possible that a majority of these internal users are actually people of Pakistani origin that moved abroad and have joined or kept membership of groups of their favored political party. Figure \ref{fig:users_map} shows the \textit{73} countries from which at least one user has joined our candidate groups.

\begin{figure}[htb]
    \centering
    \includegraphics[width=8cm]{users_map.pdf}
    \caption {\textbf{Number of Users by Geographic Location (Log Scale).} \emph{Majority of Users are located in Pakistan, India and Middle East.}}
    \label{fig:users_map}
\end{figure}
% \kiran{is it a bug that it shows 1.5k in the legend? It should be 15k i guess.}
% Elaaf: Yes, the typo has been remedied.




\subsection{Languages Used in Text Messages}
WhatsApp does not store any information regarding the language of a Text Message. However, analyzing the linguistic composition of our text messages is important. To this end, we have used Google Translate API to detect the language in a given text message. Language detection is particularly challenging as Urdu is written using both English (Roman Urdu) and Arabic (Regular Urdu) characters and distinguishing between Roman Urdu and English is difficult and error-prone. Each text messages is cleansed of special characters, emojis, and URLs.\par

\begin{figure}[hbt]
    \centering
    \includegraphics[width=8cm]{lang_texts.png}
    \caption {\textbf{Languages Used in Texts (Log Scale).}
    \emph{Urdu, Official Language of Pakistan is most used, followed by English and a few regional languages}\ignacio{is the distribution of texts across languages similar before and after covid? }}
    \label{fig:lang_texts}
\end{figure}

Only texts containing greater than or equal to 10 characters are considered for language detection. This results in around 40k texts. The results are summarized in Figure \ref{fig:lang_texts} for all languages found with a support of at least 100 text messages. Urdu being the official language of Pakistan is the most used. This includes both Arabic and Roman Urdu texts. English comes at a distant second. Followed by Hindi and other regional Pakistani languages such as Sindhi, Pushto, etc. Text messages for the languages in the lower count (Gujarati, Hindi, Pushto) are also individually inspected and it is observed that a majority of them are in fact Roman Urdu misidentified by the Google Translate API.
% \gareth{I think the language detection is something we can remove from the results section, and just have in the data section. We don't really do much with the language stuff, so safer to frame it as just a basic characterisation (rather than a key result).}





\subsection{Network Structure}
% The network structure of our joined WhatsApp groups is shown in Figure \ref{fig:group_user_graph}. Each node represents a group, with the number of users in a group indicated by the color and size of the node. Edges are defined by having one or more users common between two groups, weighted by the number of common users indicated by the color and width of the edge.\par


\begin{table}[htb]
\textbf{ \caption{ \textbf{Distribution of Users by Number of Groups joined. }\emph{93\% Users joined only 1 Group, 7\% Users joined multiple Groups} } \label{table:user_group_count} }
\begin{center}
\begin{tabular}{| c | c | }
\hline
\textbf{\#Groups Joined}  & \textbf{\#Users}  \\
\hline
1 & 15413  \\
\hline
2 & 774 \\
\hline
3 &  174 \\
\hline
4 &  54 \\
\hline
5 &  24 \\
\hline
6 &  14 \\
\hline
7 &  8 \\
\hline
8 &  3 \\
\hline
9 &  7 \\
\hline
10+ &  18 \\
\hline
\end{tabular}
\end{center}
\end{table}


\begin{figure}[hbt]
    \centering
    \includegraphics[width=8cm]{cdf_user_groups.pdf}
    \caption{ \textbf{Distribution of Users by Number of Groups joined. }
    \emph{93\% Users joined only 1 Group, 7\% Users joined multiple Groups}}
    \label{fig:cdf_user_groups}
\end{figure}




It can be observed that a few groups, affiliated with the same political party, are very closely connected with a large number of common users between them. This can be an indication of organized WhatsApp operations by the given political party. There is one major such cluster of groups and two smaller and stretched out clusters, each with their own political sides. It may be inferred that these clustered groups promote the sharing of content between them, such that a message appearing in one of the members is very likely to appear in another member group. \gareth{Interesting but we may need to dig a bit deeper here. The visualisation is difficult to read and extract a message from. We need a clear hypothesis? The main interesting one is that a small subset of users join many groups and spread misinformation. This strikes me as something that could go later on (if it's true). Maybe here, we could have a table/CDF that summarises the number of groups each user joins?}

\kiran{Agreed with Gareth. I think the more interesting part here is to see if any content is specifically shared extensively within a cluster. The figure can be removed.
Can we think of coordinated message posting? are there similar messages shared in a small set of groups?}



% \begin{figure}[htb]
%     \centering
%     \includegraphics[width=8cm]{group_user_graph.png}
%     \textbf{\caption{\textbf{Group Network.} \emph{Nodes represent Groups, Edges represent common users between groups weighted by count. Groups affiliated with the same political party tend to from highly linked clusters}}
%     \label{fig:group_user_graph}}
% \end{figure}



Table \ref{table:user_group_count} shows the distribution of users concerning the number of groups joined by them. 93\% of our observed Users have joined only a single group. This percentage may be lower in actuality, as our observed groups may not incorporate all the public groups. Only 7\% of Users are in multiple groups. This small percentage of users may be attributed for most of the inter-group content dissemination. A very few users were also observed to have joined up to 36 Groups.

==> Drafts/video.tex <==
\subsection{Video Analysis Methodology} 

Our dataset also consisted of videos shared in the WhatsApp public groups. A total of 5,170 videos were downloaded and decrypted. We sorted the videos by date and time they were sent in a group and started playing the videos in sequence. So far, we have analyzed 1,627 videos and took out 139 COVID-19 related videos.
\ignacio{I understand these are different videos, what is the distribution by the number of times they were shared? May be looking at the most shared ones would be a good choice}
%\gareth{Justify choice of this threshold}
We analyzed 1,627 videos by playing each one of them and looking at the contents in it. 
%\gareth{How were the videos spread across groups. How did you sample the 1007 videos?}
Some videos were purely news headlines so we went through all of the news in a video to see if it contains any news about COVID-19. If news about COVID-19 was found then that video was selected otherwise discarded. In the same way, we looked at all the videos. Some videos had a religious perspective about COVID-19 and told precautionary measures like practicing Ablution to keep yourself safe from the virus. These sorts of videos were also selected. Some videos talked about the financial issues being faced due to COVID-19, those videos were also selected. In short, any video which was related to COVID-19 in any form was selected. Out of these 1,354 videos we found only 139 videos that were related to COVID-19 as mentioned above and we selected these videos for further analysis.
\kiran{What were the other 900+ videos? what is the typical length of a video? Also report this number for images (how many tagged vs. how many are relevant)}








\subsubsection{Videos Analysis}

% \jq{The term infodemic is not clearly defined yet. Furthermore, in a section titled COVID-19 infodemic, all the text should be related to the infodemic phenomenon---which does not seem to be the case here. In UN/WHO's terminology, infodemic typically means an infodemic of misinformation and something that needs to be countered.}

We analyzed 139 videos related to COVID-19 about the contents they had and the type of information in them. 
%\gareth{Not sure this stands-up on its own as the final section. I would suggest integrating into the previous sections. If we only have 68 samples, it might be better suited to qualitative analysis rather than the current quantified approach.}
First we analyzed the length of videos that were shared. For that we made bins of 0 - 10 minutes, 10 - 20 minutes, and 20+ minutes. The most common length of videos was 0 - 10 minutes. Figure \ref{fig:length} shows the distribution of videos against their duration in minutes.

\begin{figure}[ht]
    \centering
    \includegraphics[width=8cm]{video_length.pdf}
    \textbf{\caption{\textbf{Duration of videos} 
    \emph{Most common bin was 0 - 10 minutes}
    }
    \label{fig:length}}
\end{figure}

\par We found three types of videos in our dataset. Simple videos, animations, and slideshows. Out of 139 COVID-19 related videos, 3 videos were slideshows, 3 videos were animations, and the rest were videos. We further divided the videos into two more categories i.e. Full and Partial. We noticed that some COVID-19 related videos did not only had information about COVID-19 but other topics as well. For example, most of the COVID-19 related videos we chose were news headlines which have news about many different things. So we categorized such videos as "Partial" because only a part of these videos was related to Coronavirus. The videos which were specifically made for COVID-19 were categorized as "Full". Out of 139 videos, 77 were categorized as "Full" and remaining 62 were categorized as "Partial".

Figure \ref{fig:themes} shows the distribution of themes in videos. Further analysis showed that most videos were edited before they were forwarded. 
%\gareth{How often were they forwarded?}
We define an edited video as a video that has been edited to add a logo, watermark, or text on it.
%\gareth{Could we quantify these edits?}
Our analysis shows that out of 139 videos 76 videos were edited; the remaining were unedited. Next, we analyzed the languages used in videos to better understand the origin of the video. Our dataset has videos in Urdu, Arabic, Punjabi, Chinese, English, Pashto, and Hindi. Figure \ref{fig:languages} shows the distribution of languages.

\begin{figure}[ht]
    \centering
    \includegraphics[width=8cm]{video_themes.pdf}
    \textbf{\caption{\textbf{Thematic Analysis of Videos.} \emph{Propagation of information is the main source of video sharing.}%\ignacio{up to now there was no ``financial'' category, I 'd merge into economics}} %\jq{You can maybe normalize by total number of videos and present in percentage terms.}
    }
    \label{fig:themes}}
\end{figure}


%\jq{I think we should avoid gratuitous graphs—which means excessively elaborate graphs for very simple data. In this example, the data can be communicated in one number: we found that 38/68 videos were edited; the remaining were unedited. We should try to improve what visualization expert Edward Tufte says the Data to Ink Ratio. Try to have more data-packed graphs. For some pointers, you may see \url{https://serialmentor.com/dataviz/} and \url{https://guides.library.duke.edu/datavis/topten}. Try to see what kinds of visualization will best work for the data we're presenting. For example, for figure 4, it might be better to use a small bar chart—like the one you have for Figure 5.}.


\begin{figure}[ht]
    \centering
    \includegraphics[width=8cm]{video_languages.pdf}
    \textbf{\caption{\textbf{Languages used in videos.} \emph{Due to COVID-19 originating in China, many related Chinese videos were shared.}%\ignacio{The distribution is quite different from the one of language in text, is this due to sampling bias?}
    }
    \label{fig:languages}}
\end{figure}

The source of a video can play an important role in determining what kind of (mis)information a video contains. Most of the videos in our dataset were just news headlines from different mainstream news channels about  COVID-19. Table \ref{fig:source_video} shows the distribution of sources.

\begin{table}[hbt]
\textbf{ \caption{ \textbf{Sources of videos} } \label{fig:source_video} }
\begin{center}
\begin{tabular}{| c | c | }
\hline
\textbf{Source}  & \textbf{\#Videos}  \\
\hline
Geo News & 41  \\
\hline
Express News & 9 \\
\hline
TikTok & 9  \\
\hline
5-Minute Crafts &  5 \\
\hline
Lahore News &  5 \\
\hline
92 News &  4 \\
\hline
ARY News &  4 \\
\hline
Dawn News &  3 \\
\hline
Youtube &  3 \\
\hline
Dawat-e-Islami &  3 \\
\hline
City Rohi &  1 \\
\hline
Vigo Video &  1 \\
\hline
Kine Master &  1 \\
\hline
Pak Asia &  1 \\
\hline
Dunya News &  1 \\
\hline
BBC Urdu &  1 \\
\hline
AlUmarNashriyat &  1 \\
\hline
Aaj News &  1 \\
\hline
Hum News &  1 \\
\hline
Din News &  1 \\
\hline
InShot &  1 \\
\hline
News One &  1 \\
\hline
Abb Tak &  1 \\
\hline
\end{tabular}
\end{center}
\end{table}



We found a total of 4 videos that were spreading misinformation regarding COVID-19. Those videos were presented out of context. A video of a bot worm removal from under the skin was portrayed as the removal of the Corona virus.  In another video, a movie trailer of “Contagion” was forwarded as COVID-19 related information, and many people forwarded this video over WhatsApp by portraying the video as an early prediction of the Novel Coronavirus. 
%\kiran{We can also automatically measure length of videos, for instance.}

==> analysis/back_seat_users.tex <==
\subsection{Active vs Back Seat WhatsApp Users}

We next proceed to explore the fraction of users who are active vs.\ inactive. Table \ref{table:dataset_overview} shows that 16,493 unique users have joined 227 WhatsApp groups. Over the entire period of our observation i.e. from January 10 to April 20, 2020 only \textbf{9,525} users have contributed one or more messages (Text, Image, etc). This indicates that overall \textbf{57.75\%} of users are \textbf{Active Users}, whereas \textbf{42.25\%} of users are \textbf{Back Seat Users}.

We can also inspect the nature of COVID-19 related information. 
Over the  period of our COVID-19 related content observation (March 16 and April 09, 2020) \textbf{1,214} users are observed to post COVID-19 related Texts. Out of these \textbf{1,214} COVID-19 related active users Texts belonging to the ``Information'' and ``Misinformation'' classes were shared by \textbf{378} and \textbf{456} users respectively. More interestingly \textbf{145} of these users are the same and they shared both ``Information'' and ``Misinformation''. \par

Another point of interest is finding the number of groups joined by users sharing COVID-19 related ``Information'' and ``Misinformation''. We observe that overall, 93\% of WhatsApp users join only a single group. A similar pattern is observed for the users sharing COVID-19 related ``Information'' and ``Misinformation'' with \textbf{89\%} and \textbf{87.8\%} of them having joined only a single group. However, for users sharing ``Information'' the highest number of groups joined by a user was \textbf{7} but for users sharing ``Misinformation'' four users joined \textbf{10}, \textbf{15} and \textbf{31} groups too. It was observed that \textbf{28\%} of users who joined multiple groups also shared Texts in multiple groups.

==> analysis/cross_grp_info_sprd.tex <==
%\subsection{Cross Group Information Spread}
Since most of the users within the network had only joined a single group. Understanding how information spreads across groups could give insights on coordinated efforts of spreading misinformation. The WhatsApp groups in our dataset majorly had political proclivity, with 127 groups openly inclined with a major political party, while the rest were political in nature but did not openly align with a political party. 
\gareth{Will this group have any additional material in? If not, we should delete it.}

==> analysis/info_spread.tex <==
\subsection{Evolution of Information over Time}

Figure \ref{fig:covid_texts_trend} shows a timeseries of the number of text messages shared over time. We clearly see that the time series ebbs and flows in response to some real-life events that trigger content sharing pertaining to that events. To dig futher into these events, we aggregate the data into time intervals of 7 days and obtain the most frequently used words in each interval. This gives us an insight on how, events like lockdowns and procedures to follow during public holidays, increased the COVID traffic.

%Table \ref{table:interval_words} shows the five most used words in descending order of their frequency in each interval.


% A peculiar trend can be observed around April 12 in Figure \ref{fig:content_trend}. Extremely few messages are shared between 9-13 April. The reason for this is unknown and this may be characterized as an anomaly as no indication of data corruption  was found. It may be due the fact that only a subset of public groups is being monitored, which might be prone to infrequent but possible activity drops. Further analysis and exploration of a larger dataset scraped over a longer period may shed further light on this.
% \ignacio{in one point to drop to 0, is th drop homogeneous across groups? could it be  a data collection issue?}
% \kiran{Are we sure it is not an error on our end? It most probably could be, especially since its close to zero messages}
% Elaaf: We have tried to confirm that this was not an error on our end. The collection device was not switched off during this period, even if it were the messages would be later received. There is also no indication of data corruption. It may be possible to explore further avenues on this issue.

% \jq{Provide a summary of the collected WhatsApp text messages in a Table presenting these statistics in one place.}
% \jq{It will be good to aim for data-rich visualizations. Much more information about your dataset can be shared. Try to design a better table so that more information about the data is shared so that our research becomes reproducible.}

